State Alignment-based Imitation Learning

Consider an imitation learning problem that the imitator and the expert have different dynamics models. Most of the current imitation learning methods fail because they focus on imitating actions. We propose a novel state alignment-based imitation learning method to train the imitator to follow the state sequences in expert demonstrations as much as possible. The state alignment comes from both local and global perspectives and we combine them into a reinforcement learning framework by a regularized policy update objective. We show the superiority of our method on standard imitation learning settings and imitation learning settings where the expert and imitator have different dynamics models.

==> sections/intro.tex <==
\section{Introduction}
\label{sec:intro}

% Imitation learning is an efficient way to teach agent to solve complicated tasks compared to learning by solely interacting with environments (reinforcement learning). 

Learning from expert demonstrations (imitation learning) is an efficient way to teach agents to solve complicated tasks.  
% While the achievements of deep reinforcement learning are exciting in having conquered many computer games (Go~\citep{AlphaGo, AlphaGoZero}, Atari games~\citep{DQN}), in practice, it still takes a large amount of trial-and-errors for these algorithms to solve complicated tasks. However, imitating expert demonstrations could be a efficient alternative for learning to perform complicated tasks which is hard for agent to learn by solely interacting with environments.  
Current imitation learning methods can be generally divided into two categories. The first one is behavioral cloning \citep{dagger} which treats the imitation learning as a supervised learning problem over state-action pairs from demonstration trajectories. 
Behavioral cloning requires the testing-time state and transition distributions to align with the distributions in demonstrations, and suffers from compounding error caused by covariate shift\citep{covar_shift_1, covar_shift_2}. 
The second category is inverse reinforcement learning \citep{irl_1, irl_2}, which tries to recover the reward function which can induce the given demonstration trajectories.
% Inverse reinforcement learning tends to be more robust than behavioral cloning (???) with a small amount of demonstration. 
GAIL\citep{gail} is a recent proposed variant of inverse RL method, and it regards the policy as a generator and trains a discriminator to match the distribution of state-action pairs generated by the policy with the distribution of state-action pairs in demonstration. GAIL alleviates the issue of compounding error, but it tends to be sample inefficient because of the reinforcement learning part in the inner loop, while behavioral cloning requires no interactions with the environment.

In addition, most of these methods rely on a common strong assumption: the expert and the imitator share the same dynamics model, i.e., they have the same action space and any feasible action has the same consequence in both agents. 
% However, GAIL does not explicitly take the completeness of task into consideration, so the agent can be stuck in a local region.%, which is similar to the "mode collapse" problem in GAN.
% \tmu{I didn't match the issues of GAIL with our tricks correspondingly, need to rethink.} In summary, most of the issues in imitation learning methods lead to a common phenomenon: \textit{the agent deviates from the demonstration trajectory during the interactions}. 
% \tmu{still need to add some analysis to these methods, so as to draw a connection between ours and them}
% Though the above mentioned imitation learning methods performs pretty well in standard imitation learning settings, but one assumption they relied on is that the expert and the imitator share the same dynamics model, i.e., they have the same action space and any feasible action has the same consequence in both agents. 
However, in real-world scenarios, the expert and the imitator would probably have different dynamics models. Imagine a robot wants to navigate through a maze with the demonstration from another robot which moves faster, it is impossible for the slow robot to imitate the actions in the demonstrations since he cannot move that fast. However, the demonstration from the fast robot is still very helpful because it shows the path to go through the maze. Traditional imitation learning methods cannot utilize the knowledge in the given demonstration, since most of them just mimic the actions.



We consider such a imitation learning problem: the agent is given several demonstration trajectories from the experts which has a different dynamics model from the agent, and the agent can also interact with the environment to improve its policy. 

Most of the traditional imitation learning methods apply some constraints on state-action pairs so as to train a policy imitating the demonstrations, e.g., behavioral cloning minimizes the total variation (?) on state-action pairs and GAIL minimizes the Jensen-Shannon divergence on state-action pairs. However, this is not feasible when the actions have different consequence in experts and imitators. To address this issue, we relax the constraints on \textit{state-action pairs} to the constraints on \textit{states}, i.e., we make the agent imitate the next state instead of the action. 


% And we want to mitigate the issue that the agent deviates from the demonstration trajectory during imitating the trajectory in the environment. This can happen in different scenarios:
% \begin{enumerate}
%     \item The environment is stochastic (initial states or transition are stochastic).
%     \item The agent reach unseen states after it executes the policy for multiple steps.
%     \item The demonstration trajectory comes from an agent whose dynamics model is different from the imitator.
% \end{enumerate}

To follow the state sequences in the given demonstrations, we guide the agent from both local and global perspectives. 

First, to prevent the agent deviating from the demonstration trajectory, it is better to have a local correcting mechanism to pull the agent back when it starts to deviate during the interactions. We propose to use $\beta$-VAE \citep{beta-vae} to generate the next state at which the agent should target, and then estimate the action by an inverse dynamics model. By using a variational autoencoder, the agent can still target at a desired next state if it deviate from the demonstration trajectory a little bit, which benefits from the latent stochastic sampling. Furthermore, give limited demonstrations, the variational lower bound will regularize VAE to act like a non-linear version of robust PCA, which will find the support of data manifold and is more robust to outliers \citep{vae_pca}.

Though VAE could help agent correct its trajectory to some extent, it only  constrain the agent's behaviour locally. GAIL minimizes Jensen-Shannon divergence between the state-action pair distributions of demonstration and imitator, so as to apply a global constraint on the agent's behaviour. 
% However, this can only constrain the 1-step behaviour (the state-action pair) of the agent.
Inspired by GAIL, we design a reward function based on the Wasserstein distance between demonstration trajectory and imitator's trajectory, and use it as a global guidance.
% , and feed this reward to agent at the end of the episode.\tmu{need to update to the new trick}
Compared to the Jensen-Shannon divergence, the Wasserstein distance also provides a better metric space where ???
% This reward can be viewed as a global constraint which tries to make the distributions of demonstration trajectory and imitator's trajectory closer. And Wasserstein distance also provides a good metric space where ???. 

% One simple way to combine the above mentioned guidance is to design a dense reward based on the local guidance and a sparse reward based on the global guidance. However, this IRL-like method is not sample-efficient. 
To combine the local and global guidance together, we propose to first pre-train the policy based the estimated action from VAE and inverse dynamics model, and further improve the policy based on the reward from the Wasserstein distance during the interactions with environment. In addition, we add to the RL objective a penalty term which is the KL divergence between the pre-trained policy and the current policy, so as to stabilize the exploration. One can view the pre-training stage as a state-based version of behavioral cloning, which targets at mimicking the next state instead of action. Therefore, our method enjoys desired properties from both behavioral cloning and GAIL, and tends to be more sample efficient than GAIL.

% \tmu{I don't how to draw an analogy between VAE trick and behavioral cloning, and ...}

% In section\ref{sec:method}, we integrated the above mentioned techniques into a novel imitation learning algorithm. 

% Furthermore, during interacting with the environment, we add a penalty term to the RL objective function to prevent the policy 
% the KL divergence between the current policy and the initial 

% If we view behavioral cloning as a direct way to train a policy, and view inverse RL or GAIL as an indirect way to train a policy. 

To empirically justify our ideas, we conduct experiments on two different settings. The first experiment setting is a traditional imitation learning setting used in GAIL, where the agent is given several demonstration trajectories and it can interact with the environment to improve its policy. The second setting is more like a transfer learning setting, where the given demonstration comes from an expert who has a different dynamics model with the imitator. In this setting, simply imitating the demonstration actions would be not sufficient to solve the task. Instead, the agent has to follow the states along the demonstration trajectory and infer the actions between them by interacting with the environment. In section ??, we compare our method with behavioral cloning and GAIL on six control tasks in Mujoco (Swimmer, Hopper, Walker2D, Ant, HalfCheetah, Humanoid) and show the superiority of our method on both of the settings.

Our contributions can be summarized as follow:
\begin{itemize}
    \item (??)Align the states instead of state-action pairs in the imitation learning problem where expert and imitator have different dynamics models.
    \item Design a novel imitation learning framework that combines local and global guidance(?)
    \item Propose to use $\beta$-VAE and Wasserstein distance to provide local and global guidance for the policy.
    
\end{itemize}
